Bulk Reconstruction from Generalized Free Fields

We propose a generalized protocol for constructing a dual free bulk theory from any boundary model of generalized free fields (GFFs). To construct the bulk operators, we employ a linear ansatz similar to the Hamilton-Kabat-Liftschytz and Lowe (HKLL) construction. However, unlike the HKLL construction, our protocol relies only on boundary data with no presupposed form for the bulk equations of motion, so our reconstructed bulk is fully emergent. For a (1+1)d bulk, imposing the bulk operator algebra as well as a causal structure is sufficient to determine the bulk operators and dynamics uniquely up to an unimportant local basis choice. We study the bulk construction for several two-sided SYK models with and without coupling between the two sides, and find good agreement with known results in the low-temperature conformal limit. In particular, we find bulk features consistent with the presence of a black hole horizon for the TFD state, and characterize the infalling fermion modes. We are also able to extract bulk quantities such as the curvature and bulk state correlators in terms of boundary quantities. In the presence of coupling between the two SYK models, we are able to observe evidence of the shockwave geometry and the traversable wormhole geometry using the two-sided mutual information between the reconstructed bulk operators. Our results show evidence that features of the geometric bulk can survive away from the low temperature conformal limit. Furthermore, the generality of the protocol allows it to be applied to other boundary theories with no canonical holographic bulk.

==> XLdef.tex <==
%\def\mathbb#1{{\rm #1}}

\def\text#1{{\rm #1}}

\def\avg#1{\left\langle#1\right\rangle}
\def\bra#1{\left\langle#1\right|}
\def\ket#1{\left|#1\right\rangle}
\def\braket#1#2{\left\langle #1\right|\left.#2\right\rangle}
\def\combin#1#2{\kc{^{#1}_{#2}}}
\def\abs#1{\left|#1\right|}
\def\kc#1{\left(#1\right)}
\def\kd#1{\left[#1\right]}
\def\ke#1{\left\{#1\right\}}
\def\Re{{\rm Re}}
\def\Im{{\rm Im}}
\def\sgn{{\rm sgn}}
\def\mode{\text{ }{\rm mod}\text{ }}
\def\trace#1{{\rm Tr}\left[#1\right]}
\def\Det#1{{\rm Det}\left(#1\right)}
\def\be{\begin{equation}}       \def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}      \def\eea{\end{eqnarray}}
\def\ba{\begin{array} }
\def\ea{\end{array} }
\def\enum#1{\begin{enumerate}#1\end{enumerate}}
\def\itmz#1{\begin{itemize}\item #1\end{itemize}}
\def\lf{\left}
\def\rt{ \right}
\def\nn{\nonumber}
\def\pa{\partial}
\def\=>{\Rightarrow}
\def\>{\rightarrow}
\def\A{\uparrow}
\def\V{\downarrow}
\def\PRB{Phys. Rev. B}
\def\PRL{Phys. Rev. Lett.}
\def\eye{\mathbb{I}}
\def\vk{{\bf k}}
\def\vp{{\bf p}}
\def\vq{{\bf q}}
\def\vr{{\bf r}}
\def\vv{{\bf v}}
\def\Tau{\mathcal{T}}
\def\Ep{\mathcal{E}}
\def\Kp{\mathcal{K}}
\def\intz{\mathbb{Z}}
\def\vect#1{\kc{\ba{c}#1\ea}}
\def\elist#1{\left\{\ba{cc} #1\ea\right.}
\def\sket#1{\left|#1\right)}
\def\sbra#1{\left(#1\right|}
\def\Cl#1#2{{\rm Cliff}^{#1,#2}}

\def\vprod#1#2{\begin{array}{ccc}&|&\\-&#1&-\\&|&\\-&#2&-\\&|&\end{array}}

\def\hprod#1#2{\begin{array}{ccccc}&|&&|&\\-&#1&-&#2&-\\&|&&|&\end{array}}


\def \red{\textcolor{red}}
\def \blue{\textcolor{blue}}

\def\addfig#1#2#3{\begin{figure}
\begin{center}
\includegraphics[width=#1]{#2}
\caption{#3
}
\end{center}
\end{figure}}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

